Clustering with fair-center representation: parameterized approximation algorithms and heuristics

We study a variant of classical clustering formulations in the context of algorithmic fairness, known as diversity-aware clustering. In this variant we are given a collection of facility subsets, and a solution must contain at least a specified number of facilities from each subset while simultaneously minimizing the clustering objective ($k$-median or $k$-means). We investigate the fixed-parameter tractability of these problems and show several negative hardness and inapproximability results, even when we afford exponential running time with respect to some parameters. Motivated by these results we identify natural parameters of the problem, and present fixed-parameter approximation algorithms with approximation ratios $\big(1 + \frac{2}{e} +\epsilon \big)$ and $\big(1 + \frac{8}{e}+ \epsilon \big)$ for diversity-aware $k$-median and diversity-aware $k$-means respectively, and argue that these ratios are essentially tight assuming the gap-exponential time hypothesis. We also present a simple and more practical bicriteria approximation algorithm with better running time bounds. We finally propose efficient and practical heuristics. We evaluate the scalability and effectiveness of our methods in a wide variety of rigorously conducted experiments, on both real and synthetic data.

==> fpt-apx-alg-2.tex <==
\begin{algorithm}
\caption{\sc $k$-MedPM$(J=((U,d),\{E_1,\cdots,E_k\},C',k),\epsilon')$}
\label{algo:kmedpm}
\KwIn{$J$, an instance of the \kmedianpm problem\\
\Indp \Indp ~$\epsilon'$, a real number}

\KwOut{$\hat{S}$, a subset of facilities}

$\hat{S} \leftarrow \emptyset$\\
\ForEach{ordered multiset $\{c'_{i_1},\cdots, c'_{i_k}\} \subseteq C'$ of size $k$} {
  \ForEach{ordered multiset $\Lambda = \{\lambda_{i_1},\cdots, \lambda_{i_k}\}$ such    that $ \lambda_{i_1} \subseteq [[\Delta]_\eta]$} {
    \For{$j=1$ to $k$} {
      $\Pi_j \leftarrow \{f \in E'_j \mid d_D(f,c'_{i_j}) = \lambda_{i_j} \}$           \label{algo:kmedpm:pi}\\
      Add a fictitious facility $F'_j$ \\
      \For{$f \in \Pi_j$} {
        $d(F'_j,f) \gets 2\lambda_{i_j}$
      }
      \For{$f \notin \Pi_j$} {
        $d(F'_j,v) \gets 2\lambda_{i_j} + \min_{f \in \Pi_j} d(f,v)$
      }
    }
    \For{$S \subseteq F$, define $\impr(S) := \textsf{cost}(C',F') -         \textsf{cost}(C',F' \cup S)$} {
      $S_{max} \leftarrow S \subseteq  \pazocal{F}$ that maximizes
      $\impr(S)$ s.t. $|S \cap \Pi_j|=1, \forall j\in[k]$\\
      \If{$\textsf{cost}(C',S_{max}) < \textsf{cost}(C',S^*)$} {
        $\hat{S} \leftarrow S$
      }
    }
  }
}
\Return $S^*$
\end{algorithm}


==> fpt-apx-alg-3.tex <==
\SetKwFor{RepTimes}{repeat}{times}{end} 

\begin{algorithm}
\caption{\sc \divkmedian-Feasibility-DP$(I= (\mathcal{E}\subseteq \{0,1\}^t, \vec{f},\vec{r}, k)$}
\KwIn{$J$, an instance of the \divkmedian problem}
\KwOut{feasibility of \divkmedian instance}


$\mathcal{E}' \leftarrow []$\\
\ForEach{$E_i \in \mathcal{E}$} {
  \RepTimes{$\min\{f(E_i),k\}$}{
    $\mathcal{E}' \leftarrow \mathcal{E}' + E_i$ \\
  }
}
$A \leftarrow [|\mathcal{E}'|, k^t]$ \\
$A[0,\vec{0}] = 0$\\
\For{$\eta \in \{0,\cdots,k\}^t$} {
  $A[0,\vec{\eta}] = 0$\\
}
\For{$i \leftarrow 1$ $\mathbf{to}$ $|\mathcal{E}'|$} {
  \For{$\eta \in \{0,\cdots,k\}^t$} {
    $A[i,\vec{\eta}] = \min\{1+A[i-1,\max(\vec{\eta} - E_i, \vec{0}]), A[i-1,\vec{\eta}]\}$\\
  }
}
\If{$A[|\mathcal{E}'|,\vec{r}] \le k$} {
  \Return \texttt{true}
}
\Return \texttt{false}
\end{algorithm}


==> improvements.tex <==
\section{Improvements}
\subsubsection{Principle of Inclusion-Exclusion}

\subsubsection{$2^{tk/2}$ using $k$-sum}
Idea: Treat the $2^t$ partition vectors as an instance of $k$-vectorsum (sum). Then, using man-in-the-middle solve it in $2^{tk/2}$ time. Note that the bounded duplicacy can also be checked while solving $2$ sum instance. (Bad idea: start with $k2^t$ vectors to bound the duplicacy!).




\subsection{Counting feasibility algorithm}
Idea: Based on FFT on $k$-SUM problem on small range.

\subsection{Bicriteria Approximations}
In this section, we study the bicriteria approximation algorithms for \divkmedian. 
\begin{definition}[$(\alpha,\beta k)$-approximation]
For $\alpha >1$ and $\beta \in \mathbb{N}$, an algorithm $\mathcal{A}$  is said to be $(\alpha,\beta k)$-approximation algorithm for \divkmedian if $\mathcal{A}$ outputs $S \subseteq \pazocal{F}$ that meets the lower bound requirement such that $|S| \le \beta k$ and $\cost(S) \le \alpha \cdot OPT$, where $OPT$ is the optimal cost of \divkmedian.
\end{definition}

\subsubsection{Warm up - Getting $(1+\sqrt{2}, 3k)$-approximation from $(3+\epsilon)$ algorithm for $d$ dimensional space $U$}
Consider the simple $(3+\epsilon)$ algorithm of Lemma~\ref{lemma:threeapx}. 
%Let $S \subseteq \pazocal{F}$ be the $3+\epsilon$ approximate solution. Now, we want to augment $k$ more facilities to $S$ to get better approximation factor. 
Recall that, for $i \in [k]$,  $\smallball_i$ is the set of facilities in $E(\vec{\gamma}_i^*)$ at a distance of equal to $\lambda_i^*$ from $c_i^*$. We showed in Lemma~\ref{lemma:threeapx}, that picking arbitrary facility $f_i \in E(\vec{\gamma}_i^*)$, for each $i \in [k]$ already gives $3$ approximation. 
Now, the intuition is that since we can pick more than one facility from each $B_i$, we can somehow smartly pick facilities that are a bit closer to $f^*_i$, if the previous ones were far. For example, consider the case when $d=2$. Then, if the picked facility $f'$ is not on the semi-circle of $B_i$ containing $f^*_i$ at its center, then the point $-f'$ lies on the semi-circle. Hence, if there is a facility at $-f'$, then $d(-f',f^*_i) \le \sqrt{2}\lambda^*_i$, which improves the approximation factor, and we pick $2$ facilities per $B_i$. However, when there is no facility at $-f'$, then we need to find the closest facility to $-f'$ that is on the semi-circle (such facility exists because $f^*_i$ lies on the semi-circle). Since $d=2$, there are two directions at $-f'$ for the closest facility. Hence, if we pick the closest facility to $-f'$ on both of its sides, then we are sure that at least one of them is on the semi-circle. Hence, we get improved approximation by picking $3$ facilities per $B_i$. However, for larger $d$, this idea does not work, and we need to figure a way to find a facility in the semi-hypersphere.
%Now, since we can pick more than $k$ facilities in the solution, for each $\smallball_i$, we will pick another $f'_i$ that is the most furthest facility from $f_i$ in $\smallball_i$. Hence, the output of the algorithm now is $S = \{f_i\}_{i \in [k]} \cup \{f'_i\}_{i \in [k]}$. Now, we will argue that when $U$ is a $d$-dimensional Euclidean space, $\cost(S) \le (1+ \sqrt{2}) \cost(S^*)$.
%The intuition is that if the chosen  facility $f_i$ was too far from $f^*_i$, then in the Euclidean ball $\smallball_i$, choosing furthest facility from $f_i$ could be much closer to $f^*_i$. This results in improvement in the approximation factor. More specifically, we show the following, that implies the desired approximation factor.

Our algorithm is as follows. For each Euclidean ball $\smallball_i$, assume that the center of $\smallball_i$ is the origin (zero vector). 
%Let $H_i$ be the half-space containing $f^*_i$ corresponding to the  hyperplane passing through origin which is orthogonal to $f^*_i$. 
Let $H_i:= \{v\in \mathbb{R}^d : \langle v,f^*_i \rangle \ge 0 \text{ and }d(c^*_i,v) = \lambda^*_i \}$ be the half-ball containing $f^*_i$. Note that for any $f \in H_i$, we have $d(f,f^*_i) \le \sqrt{2} \lambda^*_i$. 
We pick three facilities $\{f^1_i,f^2_i,f^3_i\}$ such that at least one of them is in $H_i$. Hence, for any $c \in C_i$, we have that $\min\{d(c,f^1_i),d(c,f^2_i),d(c,f^3_i)\} \le d(c,f^*_i) + \min\{d(f^*_i,f^1_i),d(f^*_i,f^2_i),d(f^*_i,f^3_i)\} \le (1 + \sqrt{2} )d(c,f^*_i)$.

The idea is very simple. First,  $f^1_i$ is any arbitrary facility from $B_i$. If $f^1_i \in H_i$, then we are done. Otherwise, pick $f^2_i$ from $B_i$ such that $\langle f^2_i, f^1_i \rangle < 0$. Note that since $f^1_i \notin H_i$, we have that $\langle f^*_i, f^1_i \rangle < 0$. And hence, we can find such $f^2_i$. Now, again, if $f^2_i \in H_i$, then we are done. Suppose $f^2_i \notin H_i$, then pick $f^3_i$ from $B_i$ such that $\langle f^3_i, f^2_i \rangle < 0$ and $\langle f^3_i, f^1_i \rangle < 0$. Such $f^3_i$ exists since both $f^1_i,f^2_i \notin H_i$, and hence $\langle f^*_i, f^2_i \rangle < 0$ and $\langle f^*_i, f^1_i \rangle < 0$.

\todo{For General $\ell_p$} I think we can get $(1+\sqrt[p]{2})$-approximation, using the above technique with $\langle a,b \rangle = ||a-b||_2$. More details required. This implies, that as $p \rightarrow \infty$, we get closer to $2$-approximation.

Now, the next lemma is very interesting. It says that we can, in fact, achieve $1+\sqrt{2}$-approximation factor even with $k$ facilities, instead of $3k$ facilities.
\begin{lemma}
Let $S:= \{f^1_i,f^2_i,f^3_i\}_{i \in [k]}$ be the set returned by the above $(1+\sqrt{2}, 3k)$-approximation algorithm. Then, there is a  \fpt algorithm $B$ that returns $S' \subseteq S$ of size $|S'| =k$ such that $\cost(S')= \cost(S)$.
\end{lemma}
\begin{proof}
The algorithm $B$ checks for every $3^k$ combinations of $k$-tupple of $S$ and outputs the one with minimum cost.
%The algorithm $B$ is a simple randomized algorithm. For every $i \in [k]$, $B$ randomly picks one $f'_i$ from $\{f^1_i,f^2,f^3_i\}$ and adds it to set $S'$. First, note that $|S'| = k$. Second, since, for every $i \in [k]$, at least one of  $\{f^1_i,f^2,f^3_i\}$ is in $H_i$, we have that $\Pr[f'_i \in H_i] \ge 1/3$. Hence, $\Pr[\forall i \in [k] f'_i \in H_i] \ge 3^{-k}$. Hence, repeating the random selection $\bigO(3^k)$ times, and choosing the minimum cost set over the repetitions, $B$ will have the desired approximation factor with constant probability.
\end{proof}

The above lemma hints about improving the $(1+2/e+\epsilon)$ algorithm using bicriteria. Let us call a bicriteria algorithm $A$ for \divkmedian a \textit{local bicriteria algorithm}, if $A$ runs the $(1+2/e+\epsilon)$ algorithm, and then adds more facilities in each $B_i$ to get improved approximation.
Formally, $A$ is \textit{$(\alpha, \beta k)$-local-bicriteria algorithm} if $A$ returns $S'= \{f_1,\cdots, f_{\beta k}\}$ then there exists $F'\subseteq S, |F'|=k$ such that $\cost(F') \le \alpha \cdot OPT$.
%Formally, let $S=\{f_i\}_{i \in [k]}$ be the output of $(1+2/e+\epsilon)$ algorithm, where $f_i \in B_i$. Then, $A$ is $(\alpha, \beta)$-local-bicriteria algorithm if $A$ returns $S'= \{f^1_i,\cdots, f^{j_i}\}_{i \in [k]}$, such that $f_i \in  \{f^1_i,\cdots, f^{j_i}\}$ and $ \{f^1_i,\cdots, f^{j_i}\} \in B_i$. 
Using the above lemma, we have the following corollary.
\begin{corollary}
	For $\alpha < 1+2/e$ and any constant $\beta$, there is no \fpt-$(\alpha, \beta k)$-local-bicriteria algorithm for \divkmedian.
\end{corollary}
\begin{proof}
	If such algorithm $A$ exists with $\alpha < 1+2/e$, then using above lemma, we get $\alpha$-\fpt-approximation algorithm with an overhead of $\bigO({\beta k \choose k})$.
\end{proof}

Hence, to get better approximation factor, we need different techniques than that we used for Euclidean space.

\subsubsection{Beating $(1+2/e+\epsilon)$-approximation using bicriteria}
In this section, we show how to get better approximation factor, if we are allowed to pick more facilities.
\begin{theorem}
	For every $\epsilon >0$, there is $(1+ \epsilon, k \log (1/\epsilon))$-\fpt-approximation algorithm for \divkmedian.
\end{theorem}
\begin{proof}
	We will prove the following lemma that is sufficient.
\begin{lemma}
	For every $\beta \ge 1$, there is $(1+\frac{2}{e^\beta}+\epsilon, \beta k)$-\fpt-approximation algorithm for \divkmedian.
\end{lemma}
\begin{proof}
	Idea: In the second for loop of Algorithm~\ref{algo:kmedpm}, in addition to creating $k$ balls $\{\Pi_j\}_{j \in [k]}$, we also create another ball $\Pi_{k+1}$ which contains copies of all facilities of  $\{\Pi_j\}_{j \in [k]}$. Further, this copied facilities have the same distance to the fictitious facilities as their corresponding facilities in $\{\Pi_j\}_{j \in [k]}$. Finally, we add another matroid constraint $|S \cap \Pi_{k+1}|= \beta k -k$ for the submodular function at line $12$.
	%Run the submodular algorithm for $\beta k$ facilities. In more detail, we repeat Algorithm~\ref{algo:kmedpm}  $\beta$ times as follows. Let $S^*_i$ be the output of Algorithm~\ref{algo:kmedpm} after iteration $i \in [\beta]$. 
	%For iteration $(i+1)$, we invoke Algorithm~\ref{algo:kmedpm} with facilities in $S^*_i$ removed, i.e., the partition set is $\{E_1 \setminus S^*_i,\cdots, E_k \setminus S^*_i\}$. Finally, the output of our algorithm $S^*$ is the union of all $S^*_i$, i.e., $S^*= \cup_{i \in [\beta]} S^*_i$.
\end{proof}	
\end{proof}

%Note that when $\beta = \log n$, then we actually recover the optimal solution.
%\begin{corollary}
%There is a \fpt algorithm for \divkmedian that returns $k \log n$ facilities $S$ such that $\cost(S) = OPT$.
%\end{corollary}

Contrasting the above result with Proposition~\ref{proposition:introduction:2}, we see that the above result is very close to the hardness result. Also, note the non-triviality of the above algorithm - Even though, we can approximate dominating set within the factor of $k \log n$ in polynomial time, which means, we can find a set of $k \log n$ facilities that meet the lower bound requirements, it is not clear how to find one such set that achieves the optimal cost. However, the above corollary shows how to find one such set in \fpt time w.r.t. $t$ and $k$.

Another observation that we would like to make is that a similar technique can be used to solve \kmedian problem with $k \log n$ facilities. And then, we find another $k \log n$ facilities that meet the lower bound requirements in polynomial time. Thus, we can solve \divkmedian with $2k \log n$ facilities in \fpt time w.r.t $k$. The above corollary says that if we are allowed to have \fpt time w.r.t. $k$ and $t$ both, then we can actually solve \divkmedian optimally with $k \log n$ facilities. It is, however, not clear to us that whether \divkmedian can be solved with $k\log n$ facilities but in \fpt  w.r.t $k$ only. On the other hand, our study shows that, even though \divkmedian is amalgamation of two hard problems, it behaves similarly from algorithmic perspective as \kmedian, when allowed to use running time additionally depending upon $t$. First, it achieves the same \fpt-approximation factor, and second, it can be solved optimally with $k \log n$ facilities. Thus, it seems like, with additional running time depending on $t$, we can smartly solve both the hard problems simultaneously, to achieve the same bounds as \kmedian.


\subsubsection{Bicriteria approximations for free}
If our instance is feasible, we know we can obtain a feasible solution
containing $O(k\log n)$ facilities in polynomial time. This is due to
the $H_n$ approximation of constrained set multicover by Vazirani
(check his book or \cite{rajagopalan1998primal}).

On the other hand, there is a bicriteria approximation algorithm for
$k$-median, achieving a $(1+O(\epsilon))$-approximation by opening
$O(k\log(1/\epsilon))$ facilities \url{https://cstheory.stackexchange.com/questions/49107/is-there-any-bi-criteria-ptas-for-metric-k-median}. 

So we can get a $\left(1+\epsilon, O\left(\log n + \log(1/\epsilon)\right)\right)$ PTAS for free.

Note: any polynomial-time bicriteria approximation requires at least $k\log n$ due to the set cover conjecture.

\section{Overview of bicriteria results}
\centering
\begin{tabular}{|r|c|c|}
\hline  & Poly time & FPT time  \\ \hline 
  $k$-median & $1+\epsilon, O(k \log(1/\epsilon))$ &  $1+\epsilon, k\log n$   \\ \hline 
  \divkmedian & $1+\epsilon, O(k\log n + k\log(1/\epsilon))$ & $1+\epsilon, k\log (1/\epsilon)$ \textcolor{red}{New!}  \\ \hline  
\end{tabular}


%%%%%%%%%%%%%% OLD WRITE UP %%%%%%%%%%%%%%
\iffalse
Let $H_i$ be the half-space containing $f^*_i$ corresponding to the  hyperplane passing through origin which is orthogonal to $f^*_i$. Let $S^{d-1}_i := \smallball_i \cap H_i$ be the half-ball containing $f^*_i$. Note that for any $f \in B'_i$, we have $d(f,f^*_i) \le \sqrt{2} \lambda^*_i$. 
Now, we pick two facilities $f_i,f'_i \in \smallball_i$ such that $d(f_i,f'_i) =2 \lambda^*_i$. If such pair exists, then note that either $f_i \in B'_i$ or $f'_i \in B'_i$ since $f'_i = -f'_i$. Hence, $\min\{d(c,f_i),d(c,f'_i) \} \le \sqrt{2}\lambda^*_i$, for $c \in C_i$.

Suppose such pair does not exist. Then, our idea is to reduce the dimension and recurse, until $d=2$. For the base case when $d=2$, let $B^2_i$ be the circle, and
$S^2_i$ be the semi-circle such that $f^*_i$ lies on the center of arc $S^2_i$. Now, if $\exists f \in B^2_i$ such that $-f \in B^2_i$, then we pick both $f$ and $-f$, we know that either $f \in S^2_i$ or $-f \in S^2_i$. Hence, we get the claimed approximation factor with $2$ facilities for $B^1_i$. Suppose not, then let $f \in B^1_i$ be an arbitrary facility. Let $v = -f$ be a point in $\mathbb{R}^2$, but no facility exists at $v$. Now, consider two closest facilities $\{f^+_i,f^-_i\}$ to $v$ such that $\langle f^+_i, v \rangle >0$ and $\langle f^-_i, v \rangle <0$. Finally, we pick $\{f,f^+_i,f^-_i\}$ as our solution. Note that it must hold that if $f \notin B^1_i$ then either $f^+_i \in B^2_i$ or $f^-_i \in B^2_i$, since $f^*_i \in B^2_i$.

Now, consider when $d >2$. If no \textit{good pair} exists in $B^d_i$, then  consider any $f \in B^d_i$ \footnote{Note that $B^d_i$ is actually of $d-1$ dimension.}, and let $v=-f$ be a point in $\mathbb{R}^d$ with no facility. We pick $f$ in our solution. Also, assume that $f \notin S^d_i$, and hence, $v \in S^d_i$. Now consider the ball $B^{d-1}_i$ centered at $v$ of radius $\sqrt{2}\lambda^*_i$ on the surface of $B^d_i$. Observe that since $v \in S^d_i$, we have $d(v,f^*_i) \le \sqrt{2} \lambda^*_i$, and hence $f^*_i \in B^{d-1}_i$. Thus, we have now reduced the dimension of the search space by one.


For each $f^*_i$, let $H_i$ be the 
For each Euclidean ball $\smallball_i$, let $B'_i$ be the half ball containing $f^*_i$ such that 

 we pick two facilities $f_i,f'_i \in \smallball_i$ such that $d(f_i,f'_i)=2\lambda^*_i$.
\begin{lemma}
For $i \in [k]$ and $c \in C_i$,
\[
\min\{ d(c,f_i), d(c,f'_i)\} \le (1 + \sqrt{2}) d(c,f^*_i)
\]
\end{lemma}
\begin{proof}
 Fix $i \in [k]$. We will show that $\min\{d(f_i,f^*), d(f'_i,f^*)\} \le \sqrt{2}\lambda^*_i$. Note that this is sufficient since, for any $c \in C_j$
 \[
 d(c,S) \le d(c,f^*_i) +  \min\{d(f_i,f^*), d(f'_i,f^*)\} \le  d(c,f^*_i) + \sqrt{2}\lambda^*_i \le (1 + \sqrt{2}) d(c,f^*_i).
 \]
 To show $\min\{d(f_i,f^*), d(f'_i,f^*)\} \le \sqrt{2}\lambda^*_i$, without loss of generality, we assume that $c^*_i = (0,\cdots,0)$ and $f^*_i = (\lambda^*_i,0,\cdots,0)$. 
 Let $B'_i := \{f \in \smallball_i: d(f,f^*_i) \le \sqrt{2} \lambda^*_i\}$. Then, if $f_i \in B'_i$, then $d(f_i,f^*) \le \sqrt{2}\lambda^*_i$, and we are done. Hence, assume that $f_i \notin B'_i$.
\end{proof}

\fi










==> tikz/tikz-defs.tex <==
\tikzstyle{exedge}  = [draw = black, ultra thick, text=black]
\tikzstyle{exedget} = [draw = yafcolor5!20, thick, text=black!20]
\tikzstyle{exedgedir} = [draw = yafcolor5!20, thick, text=black!20, latex-latexnew, arrowhead=5mm]

\tikzstyle{exnode}  = [thick, draw = black, fill=yafcolor2!05, font = \large,  circle, inner sep = 1pt, text=black, minimum width=14pt]
\tikzstyle{exnodet} = [thick, draw = yafcolor4!20, fill=yafcolor2!02, font = \large,  circle, inner sep = 1pt, text=black!20, minimum width=14pt]
\tikzstyle{exlabel} = [circle, inner sep = 1pt,  font = \large, text = black, auto]
\tikzstyle{exsource}  = [thick, draw = red, fill=yafcolor2!05, font =\large, inner sep = 1pt, text=black, minimum width=14pt, minimum height=14pt]
\tikzstyle{exsquare}  = [thick, draw = yafcolor4!20, fill=yafcolor2!05, font =\large, inner sep = 1pt, text=black, minimum width=14pt, minimum height=14pt]
\tikzstyle{exdiamond}  = [thick, draw = yafcolor4!20, fill=yafcolor2!05, font =\large, inner sep = 1pt, diamond, text=black, minimum width=18pt, minimum height=18pt]

\tikzstyle{label}  = [fill=white, minimum width=0pt, inner sep = 0pt]


\tikzstyle{node1}  = [thick, draw = yafcolor1!100, fill=yafcolor1!05, circle, inner sep = 2.8pt]
\tikzstyle{node2}  = [thick, draw = yafcolor2!100, fill=yafcolor2!05, circle, inner sep = 2.8pt]
\tikzstyle{node3}  = [thick, draw = yafcolor3!100, fill=yafcolor3!05, circle, inner sep = 2.8pt]
\tikzstyle{node4}  = [thick, draw = yafcolor4!100, fill=yafcolor4!05, circle, inner sep = 2.8pt]
\tikzstyle{node5}  = [thick, draw = yafcolor5!100, fill=yafcolor5!05, circle, inner sep = 2.8pt]
\tikzstyle{node7}  = [thick, draw = yafcolor7!100, fill=yafcolor7!05, circle, inner sep = 2.8pt]
\tikzstyle{node8}  = [thick, draw = yafcolor8!100, fill=yafcolor8!05, circle, inner sep = 2.8pt]


\tikzstyle{node}  = [thick, draw = black!100, fill=yafcolor2!05, font = \large,  circle, inner sep = 1pt, text=black, minimum width=14pt]
\tikzstyle{mnode}  = [thick, draw = black!100, fill=yafcolor2!05, font = \large,  circle, inner sep = 1pt, text=black, minimum width=10pt]

\tikzstyle{fcircle}  = [thick, draw = black!100, font = \large,
circle, inner sep = 1pt, text=black, minimum width=4cm]
\tikzstyle{dcircle}  = [loosely dotted, ultra thick, draw = red, font = \large,
circle, inner sep = 1pt, text=black, minimum width=4cm]

\tikzstyle{point1}  = [draw = yafcolor1!100, fill=black, circle, inner sep=2pt]
\tikzstyle{point2}  = [draw = red, fill=red, circle, inner sep=2pt]

